Benchmarking Egocentric Multimodal Goal Inference for Assistive Wearable Agents

There has been a surge of interest in assistive wearable agents: agents embodied in wearable form factors (e.g., smart glasses) who take assistive actions toward a user's goal/query (e.g. "Where did I leave my keys?"). In this work, we consider the important complementary problem of inferring that goal from multi-modal contextual observations. Solving this "goal inference" problem holds the promise of eliminating the effort needed to interact with such an agent. This work focuses on creating WAGIBench, a strong benchmark to measure progress in solving this problem using vision-language models (VLMs). Given the limited prior work in this area, we collected a novel dataset comprising 29 hours of multimodal data from 348 participants across 3,477 recordings, featuring ground-truth goals alongside accompanying visual, audio, digital, and longitudinal contextual observations. We validate that human performance exceeds model performance, achieving 93% multiple-choice accuracy compared with 84% for the best-performing VLM. Generative benchmark results that evaluate several families of modern vision-language models show that larger models perform significantly better on the task, yet remain far from practical usefulness, as they produce relevant goals only 55% of the time. Through a modality ablation, we show that models benefit from extra information in relevant modalities with minimal performance degradation from irrelevant modalities.

==> misc_results.tex <==

\textbf{Context window duration.}
% TODO(pedro): do also on generative for completion
% TODO(pedro): plot with modalities and durations axis swapped might be better
For this analysis, we fixed input modalities to audio and vision (VA) as these performed the best overall and are arguably the most relevant for context windows.
As illustrated in Figure~\ref{fig:breakdown_durations}, context window durations did not exhibit any notable influence on MCQ performance, aside from: (i) higher robustness to context window durations on the large model ensemble, (ii) VD and VADL data slices being the most sensitive to context window durations on both ensembles, and (iii) data slice VADL increasing larger models' performance in longer duration settings.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.49\linewidth]{figures/breakdown_durations_small.pdf}
    \includegraphics[width=0.49\linewidth]{figures/breakdown_durations_large.pdf}
    \caption{Performance breakdown on the MCQ task for VA input modalities, according to context window durations and data slices, for small and large model ensembles (left and right, respectively).}
    \label{fig:breakdown_durations}
\end{figure}

    
\textbf{Distractor Similarity.}
Similarly to above, we fixed input modalities to audio and vision (VA) for this analysis.
We observe small decreases in MCQ performance across all models between low and high distractor similarity settings (see Figure~\ref{fig:breakdown_lures}), with qwen-72b scoring the highest in the both settings (90\% and 85\% for the low and high distractor similarity settings, respectively). The performance for the other models was not much different from qwen-72b, except for llama3.2v which scored the lowest at (53\% and 50\%  for the low and high distractor similarity settings, respectively). Figure~\ref{fig:breakdown_lures_ensembles} breaks down MCQ performance per input modalities among small and large models. 
% TODO(Pedro): Interestingly, we observe a notable decrease in accuracy when increasing distractor similarity for data slice VADL, while the remaining data slices decreased marginally. Aside from the larger error bars due to the small data slice volume, we hypothesize that 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/breakdown_lures.pdf}
    \caption{Performance breakdown on the MCQ task for VA input modalities, according to distractor similarity.}
    \label{fig:breakdown_lures}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.49\linewidth]{figures/breakdown_lures_small.pdf}
    \includegraphics[width=0.49\linewidth]{figures/breakdown_lures_large.pdf}
    \caption{Performance breakdown on the MCQ task for VA input modalities, according to distractor similarity for the small (left) and large (right) model ensembles.}
    \label{fig:breakdown_lures_ensembles}
\end{figure}

